Dualities in Multiparameter Persistence

In the theory of persistent homology, a well known duality relates the barcodes of the absolute homology and relative cohomology of a one-parameter simplicial filtration. Motivated by the problem of computing free presentations of the (co)homology of multiparameter Rips filtrations, we give a multiparameter generalization of this duality. Considering two duality functors on multiparameter persistence modules, the pointwise dual $(-)^*$ and the global dual $(-)^\dagger$, we show that $H_q(C)^* \cong H^{N+q}(C^\dagger)$ for chain complexes $C$ of free $N$-parameter persistence modules with acyclic colimit. We give an elementary and accessible proof based on a long exact sequence argument, and also give an alternate proof that casts the result as a special case of multigraded Grothendieck local duality. As a corollary, we recover a simple correspondence between minimal free resolutions of a persistence module $M$ and those of its pointwise dual $M^*$, a result previously obtained by Miller, 2000. These results form the foundation of a state-of-the-art algorithm for computing free resolutions of the homology of Vietoris--Rips bifiltrations, described in a forthcoming paper.

==> modules.tex <==

% Commands for drawing diagrams of 2-parameter persistence modules
\usepackage{xstring}
\usetikzlibrary{shapes, shapes.misc, backgrounds}

\tikzset{%
	on layer/.code={%
		\pgfonlayer{#1}\begingroup
		\aftergroup\endpgfonlayer
		\aftergroup\endgroup
}}

% Size of the symbols for generators, relations and 2-syzygies.
\newlength{\ModuleDiagramSymbolSize}
\setlength{\ModuleDiagramSymbolSize}{.2ex}

% Styles for module diagrams.
\tikzset{%
	really densely dotted/.style={line cap=round, dash pattern=on 0pt off 2\pgflinewidth},
	% Styles for the depiction of 0-, 1- and 2-syzygies
	module diagram symbol size/.style={%
		generator/.style={shape=circle, fill, outer sep=0, inner sep=#1},
		coordinate/.style={shape=circle, draw, outer sep=0, inner sep=#1},
		relation/.style={shape=diamond, fill, outer sep=0, inner sep=#1},
		syzygy/.style={shape=cross out, draw, outer sep=0, inner sep=#1}
	},
	every module diagram/.style={},
	every module/.style={line width=0.5pt},
%	{every module diagram/.append style={x=2mm, y=2mm, every label/.append style={label distance=0pt, inner sep=0pt}}}
	% Style for module diagrams
	module diagram/.style={%
		x=3mm,
		y=3mm,
		module diagram symbol size=.2ex,
		line cap=round,
		every label/.append style={%
			font=\scriptsize,
			label distance=1pt,
			inner sep=0pt,
		},
		every module diagram
	},
	% Dotted style used for 'extended' lines
	xdotted/.style={dash pattern=on 0pt off 1.5pt},
	diagram fill/.style={fill opacity=0.2},
	diagram transform/.style={shift={(-.5,-.5)}},
	invisible/.style={opacity=0, diagram fill/.style={opacity=0}}
}

% Draws an integer grid with gray dots
% Example: \Grid[from-x](step-x){to-x}[from-y](step-y){to-y}
\ProvideDocumentCommand{\Grid}{O{0} D(){0.5} m O{0} D(){0.5} m}{%
	\begin{scope}[on background layer]
		\foreach \i in {#1, #2, ..., #3}{
			\foreach \j in {#4, #5, ..., #6}{
				\fill[gray] (\i, \j) circle (0.5pt);
			}
		}
	\end{scope}
}

% Draws a coordinate axes. The origin is given by the second parameter
% Example: \Axes(from)[cross](to)
\NewDocumentCommand{\Axes}{O{->, shorten >=-0pt} r() O{0,0} r()}{%
	\coordinate (ninf) at (#2);
	\coordinate (O) at (#3);
	\coordinate (inf) at (#4);
	\draw[#1] (ninf -| O) -- (O |- inf);
	\draw[#1] (ninf |- O) -- (O -| inf);
	\coordinate (inf) at (#4);
}

% Coordinate axes with a dotted 'gap' to indicate that something has been cut off
% Example: \ExtendedAxes(from)[cross]{start dots}{stop dots}(to)
\NewDocumentCommand{\ExtendedAxes}{r() O{0,0} m m r()}{%
	\coordinate (ninf) at (#1);
	\coordinate (O) at (#2);
	\coordinate (inf) at (#5);
	\coordinate (startdots) at (#3);
	\coordinate (enddots) at (#4);
	\draw (ninf -| O) -- (O |- startdots);
	\draw[xdotted] (O |- startdots) -- (O |- enddots);
	\draw[->, shorten >=-4pt] (O |- enddots) -- (O |- inf);
	\draw (ninf |- O) -- (O -| startdots);
	\draw[xdotted] (O -| startdots) -- (O -| enddots);
	\draw[->, shorten >=-4pt] (O -| enddots) -- (O -| inf);
}

% Depicts a free (or flat) module generated at #2, drawn with style #1, and draws a \node[#1,#3]{#4} at #2.
\NewDocumentCommand{\FreeModule}{D<>{} O{} r() O{} m}{%
	\begin{scope}[#2]
		\node[#4] at (#3) {#5};
		\coordinate (n) at (#3);
		\coordinate (n) at ([diagram transform]n);
		\IfSubStr{#1}{x}{\coordinate (n) at (ninf |- n);}{}
		\IfSubStr{#1}{y}{\coordinate (n) at (ninf -| n);}{}
		\begin{scope}[on background layer=#2]
			\fill[diagram fill] (n) rectangle (inf);
		\end{scope}
		\IfSubStr{#1}{x}{}{\draw (n) -- (n |- inf);}
		\IfSubStr{#1}{y}{}{\draw (n) -- (n -| inf);}
	\end{scope}
}

% Same, but draws a dotted gap for both axes.
\NewDocumentCommand{\xyExtendedFreeModule}{O{} r() O{} m}{%
	\begin{scope}[every module, #1]
		\path (#2) node[#3] {#4} coordinate (n);
		\begin{scope}[on background layer=#1]
			\fill[diagram fill] (#2) rectangle (inf);
		\end{scope}
		\draw
			(n) -- (n |- startdots)
			(n |- enddots) -- (n |- inf)
			(n) -- (n -| startdots)
			(n -| enddots) -- (n -| inf);
		\draw[xdotted]
			(n |- startdots) -- (n |- enddots)
			(n -| startdots) -- (n -| enddots);
	\end{scope}
}

% Same, but draws a dotted gap for the x-axis.
\NewDocumentCommand{\xExtendedFreeModule}{O{} r() O{} m}{%
	\begin{scope}[#1]
		\path (#2) node[#3] {#4} coordinate (n);
		\begin{scope}[on background layer=#1]
			\fill[diagram fill] (#2) rectangle (inf);
		\end{scope}
		\draw
			(n |- inf) -- (n) -- (n -| startdots)
			(n -| enddots) -- (n -| inf);
		\draw[xdotted]
		(n -| startdots) -- (n -| enddots);
	\end{scope}
}

% Same, but draws a dotted gap for the y-axis.
\NewDocumentCommand{\yExtendedFreeModule}{O{} r() O{} m}{%
	\begin{scope}[#1]
		\path (#2) node[#3] {#4} coordinate (n);
		\begin{scope}[on background layer=#1]
			\fill[diagram fill] (#2) rectangle (inf);
		\end{scope}
		\draw
		(n -| inf) -- (n) -- (n |- startdots)
		(n |- enddots) -- (n |- inf);
		\draw[xdotted]
		(n |- startdots) -- (n |- enddots);
	\end{scope}
}

% Draws the complement of a free module generated at #2 with style #1.
\NewDocumentCommand{\FreeComplement}{O{} r() O{} m}{%
	\begin{scope}[#1]
		\path (#2) node[#3] {#4} coordinate (n);
		\coordinate (n) at ([shift={(-.5,-.5)}]n);
		\begin{scope}[on background layer=#1]
			\fill[diagram fill] (n |- inf) |- (n -| inf) |- (ninf) |- (inf -| n);
		\end{scope}
		\draw (n |- inf) |- (n -| inf);
	\end{scope}
}

% Draws an injective module 'generated' at #2 with style #1.
\NewDocumentCommand{\InjModule}{D<>{} O{} r() O{} m}{%
	\begin{scope}[every module, #2]
		\node[#4] at (#3) {#5};
		\coordinate (n) at (#3);
		\coordinate (n) at ([shift={(.5,.5)}]n);
		\IfSubStr{#1}{x}{\coordinate (n) at (inf |- n);}{}
		\IfSubStr{#1}{y}{\coordinate (n) at (inf -| n);}{}
		\begin{scope}[on background layer=#2]
			\fill[diagram fill] (n) rectangle (ninf);
		\end{scope}
		\IfSubStr{#1}{x}{}{\draw (n) -- (n |- ninf);}
		\IfSubStr{#1}{y}{}{\draw (n) -- (n -| ninf);}
	\end{scope}
}

% Draws the complement of an injective module 'generated' at #2 with style #1.
\NewDocumentCommand{\InjComplement}{O{} r() O{} m}{%
	\begin{scope}[every module, #1]
		\path (#2) node[#3] {#4} coordinate (n);
		\coordinate (n) at ([shift={(-.5,-.5)}]n);
		\begin{scope}[on background layer=#1]
			\fill[diagram fill] (ninf |- n) -| (n |-  ninf) -| (inf) -| cycle;
		\end{scope}
		\draw (ninf |- n) -| (n |-  ninf);
	\end{scope}
}

% Same, but truncates the module at infinity and draws a dotted gap.
% The starred version draws the syzygies.
\NewDocumentCommand{\TruncatedInjModule}{s O{} r() O{} m}{%
	\begin{scope}[every module, #2]
		\coordinate (n) at (#3);
		\IfBooleanTF{#1}{
			% Version with star: draw the grades
			\path
			(ninf) node[generator] {}
			(ninf |- n) node[relation] {}
			(ninf -| n) node[relation] {}
			(n) node[syzygy, #4] {#5};
		}{
			\node[#4, at=(n)] {#5};
		}
		\begin{scope}[on background layer=#2]
			\fill[diagram fill] (#3) rectangle (ninf);
		\end{scope}
		\draw
			(n |- enddots) |- (n -| enddots)
			(n |- startdots) |- (enddots |- ninf)
			(startdots |- ninf) -| (startdots -| ninf)
			(enddots -| ninf) |- (startdots |- n);
		\draw[xdotted]
			 (n -| enddots) -- (n -| startdots)
			(startdots -| n) -- (enddots -| n)
			 (enddots |- ninf) -- (startdots |- ninf)
			(startdots -| ninf) -- (enddots -| ninf);
	\end{scope}
}

% Same, but truncates the module at infinity and draws a dotted gap.
% The starred version draws the syzygies.
\NewDocumentCommand{\TruncatedInjComplement}{s O{} r() O{} m}{%
	\begin{scope}[#2]
		\coordinate (n) at (#3);
		\IfBooleanTF{#1}{
			% Version with star: draw the grades
			\path
				(ninf |- n) node[generator] {}
				(ninf -| n) node[generator] {}
				(n) node[relation, #4] {#5};
		}{
			\node[#4, at=(n)] {#5};
		}
		\begin{scope}[on background layer=#2]
			\fill[diagram fill] (n) -- (ninf |- n) -- (ninf |- inf) -- (inf) -- (ninf -| inf) -- (n |- ninf) -- cycle;
		\end{scope}
		\draw
			(inf -| ninf) -- (ninf |- n) -- (startdots |- n)
			(enddots |- n) -| (n |- enddots)
			(n |- startdots) -- (n |-  ninf) -- (ninf -| inf);
		\draw[xdotted]
			(startdots -| n) -- (enddots -| n)
			(startdots |- n) -- (enddots |- n);
	\end{scope}
}

% Usage: \StepModule[green](0,3){-| (1,2) -| (2,1)}(3,0)
\NewDocumentCommand\StepModule{O{}r()mr()}{%
	\draw[#1] (inf -| #2) -- (#2) #3 -| (#4) -- (#4 -| inf);
	\begin{scope}[on background layer=#1]
		\fill[diagram fill] (inf -| #2) -- (#2) #3 -| (#4) -- (#4 -| inf) |- cycle;
	\end{scope}
}

==> preamble.tex <==
\makeatletter
\usepackage{mathtools,amssymb,amsfonts,nicematrix,mleftright,bm,./mysansmath,accents,xstring,etoolbox,tikz,array,booktabs,csquotes,microtype,subcaption,xpatch,placeins,multirow,graphicx}
\usepackage[shortcuts]{extdash}
\usepackage[date=year]{biblatex}
\usepackage[textsize=tiny,format=textsf]{todonotes}
\usepackage[shortcuts]{extdash}
\usepackage[font=small]{caption}
% BEGIN_FOLD cross-references
\colorlet{darkgreen}{green!40!black}
%\usepackage{zref-clever}
\usepackage{hyperref,amsthm}
\hypersetup{colorlinks=true,urlcolor=blue,citecolor=darkgreen,linkcolor=darkgreen,linktocpage,bookmarksnumbered,unicode}
\usepackage[patch-newtheorem]{./mytheorem-enum}

% Patch new amsmath-subcaption-conflict https://tex.stackexchange.com/a/746030/27717
\patchcmd\caption@subtypehook{\let\label\subcaption@label}
{\let\label\subcaption@label\let\ltx@label\subcaption@label}{}{\fail}

% Reference math with cleveref
\usepackage[capitalize]{cleveref}
\crefname{equation}{}{}
\Crefname{equation}{}{}
\crefname{page}{page}{pages}
\Crefname{page}{Page}{Pages}

% END_FOLD
% BEGIN_FOLD acronyms
\newcommand{\ie}{i.e.}
\newcommand{\ia}{i.a.}
\newcommand{\eg}{e.g.}
\newcommand{\ip}{i.p.}
\newcommand{\wrt}{with respect to}
\newcommand{\sth}{such that}
\newcommand{\textiff}{iff}
\newcommand{\PH}{persistent homology}
\newcommand{\PC}{persistent cohomology}
\newcommand{\PHC}{persistent (co)homology}
\newcommand{\GM}{\textsc{gm}}
\newcommand{\MFR}{MFR}
\newcommand{\TDA}{\textsc{tda}}
\newcommand\SFD{\textsc{sfd}}
% END_FOLD
% BEGIN_FOLD mathematical symbols
% Arrows
\let\into\hookrightarrow
\let\onto\twoheadrightarrow
\let\xto\xrightarrow
\let\xinto\xhookrightarrow
\let\xonto\xtwoheadrightarrow
\providecommand\mapsfrom{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
\providecommand{\mapstofrom}{%
	\mathrel{\ooalign{%
		\raise.4ex\hbox{$\hskip.2ex\mapsto$}\cr%
		\raise-.4ex\hbox{$\mapsfrom\hskip.2ex$}\cr}%
	}%
}
% Double struck brackets from stmaryrd
\DeclareSymbolFont{stmry}{U}{stmry}{m}{n}
\DeclareMathDelimiter\llbracket{\mathopen}{stmry}{"4A}{stmry}{"71}
\DeclareMathDelimiter\rrbracket{\mathclose}{stmry}{"4B}{stmry}{"79}
% Number sets
\newcommand{\R}{\mathbf{R}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\ZZ}{\mathbf{Z}^2}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\IntSet}[1]{\llbracket#1\rrbracket}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\m}{\mathfrak{m}}
% Categories
\newcommand{\Vect}{\mathbf{Vec}}
\newcommand{\vect}{\mathbf{vec}}
\newcommand{\Simp}{\mathbf{Simp}}
\newcommand{\simp}{\mathbf{simp}}
\newcommand{\gMod}[1]{#1\mhyphen\mathbf{gMod}}
\newcommand{\gmod}[1]{#1\mhyphen\mathbf{gmod}}
\newcommand{\Pers}[1]{#1\mhyphen\mathbf{Pers}}
\newcommand{\pers}[1]{#1\mhyphen\mathbf{pers}}
\newcommand{\FiltSimp}[1]{\mathrm{Simp}^{\subseteq #1}}
\newcommand{\Db}{\mathcal{D}^\mathrm{b}}
\newcommand{\Kb}{\mathcal{K}^\mathrm{b}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\DbP}{\Db(\Pers{\ZZ})}
\newcommand{\Perf}[1]{\mathbf{perf}_{\Pers{#1}}}
\newcommand{\Proj}[1]{\mathcal{P}_{#1}}
\newcommand{\Inj}[1]{\mathcal{I}_{#1}}
\newcommand{\one}{\bm{1}}
\newcommand{\Infty}{\bm{\infty}}
\newcommand{\uZ}{\smash{\overline{\Z}}\vphantom{\Z}}%
\newcommand{\lZ}{\underline{\Z}}%
% Functions and functors
\newcommand{\VR}{\mathit{VR}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\Ext}{\mathrm{Ext}}
\newcommand{\IHom}{\mathsf{Hom}}
\newcommand{\IExt}{\mathsf{Ext}}
\DeclareMathOperator{\tot}{tot}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\dom}{domain}
\DeclareMathOperator{\codom}{codomain}
\let\lim\relax
\DeclareMathOperator{\Ch}{\mathbf{Ch}}
\DeclareMathOperator{\lim}{lim}
\DeclareMathOperator{\argmax}{arg\,max}
\DeclareMathOperator{\injdim}{inj\,dim}
\DeclareMathOperator{\piv}{piv}
\DeclareMathOperator{\Lim}{Lim}
\DeclareMathOperator{\Colim}{Colim}
\DeclareMathOperator{\xColim}{xColim}
\DeclareMathOperator{\yColim}{yColim}
\DeclareMathOperator{\lpiv}{l-piv}
\DeclareMathOperator{\cpiv}{c-piv}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\barc}{barc}
\DeclareMathOperator*{\toplus}{\textstyle\bigoplus}
\newcommand\Mat[1]{\mathsfit{#1}}
\newcommand{\op}{{\mathrm{op}}}
\renewcommand{\d}{\delta}
\DeclareMathOperator{\id}{id}
\newcommand{\Id}{I}
\newcommand{\FF}{\Bbbk}
\newcommand{\SimpleModule}{\mathbf{k}}
\renewcommand{\underbar}[1]{\underaccent{\bar}{#1}}
\let\vec\bm
% Graded matrices
\DeclareMathOperator{\rg}{rg}
\DeclareMathOperator{\cg}{cg}
\newcommand{\uMat}[1]{\mathsf{u}(#1)}
% lex/colex relations
\newcommand{\lex}[1]{#1_{\mathrm{lex}}}
\newcommand{\colex}[1]{#1_{\mathrm{colex}}}
\newcommand{\phrel}[1]{\mathrel{\phantom{#1}}}
% Others
\mathchardef\mhyphen="2D
% Paired delimiters; usage: \Set{x; P(x)} and \Span{x; P(x)}
\DeclarePairedDelimiter{\Shift}{\langle}{\rangle}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiterX{\Set}[1]{\{}{\}}{\setargs{#1}}
\DeclarePairedDelimiterX{\Span}[1]{\langle}{\rangle}{\setargs{#1}}
\NewDocumentCommand{\setargs}{>{\SplitArgument{1}{;}}m}{\setargsaux#1}
\NewDocumentCommand{\setargsaux}{mm}{\IfNoValueTF{#2}{#1} {#1\nonscript\:\delimsize\vert\allowbreak\nonscript\:\mathopen{}#2}}%

% Matrices: Type \Mtx{...} for a matrix in small print. Also available: \Mtx[\big]{...}, \Mtx*[c][\big]{...}
\NewDocumentCommand{\Mtx}{s}{\IfBooleanTF{#1}{\@MtxStar}{\@Mtx}}
\NewDocumentCommand{\@Mtx}{om}{%
	\IfNoValueTF{#1}{%
		\mleft(\begin{smallmatrix}#2\end{smallmatrix}\mright)
	}{%
		\mathopen#1(\begin{smallmatrix}#2\end{smallmatrix} \mathclose#1)
	}
}
\NewDocumentCommand{\@MtxStar}{O{c}om}{%
	\IfNoValueTF{#2}{%
		\mleft(\begin{smallmatrix*}[#1]#3\end{smallmatrix*}\mright)
	}{%
		\mathopen#2(\begin{smallmatrix*}[#1]#3\end{smallmatrix*} \mathclose#2)
	}
}
\newcommand{\Stack}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

% Scriptsize case distinction
\newenvironment{smallcases}{\left\{\begin{smallmatrix*}[l]}{\end{smallmatrix*}\right.}
\newenvironment{smalllrcases}{\left\{\begin{smallmatrix*}[l]}{\end{smallmatrix*}\right\}}

% scaling vdots (https://tex.stackexchange.com/a/246695/27717)
\DeclareRobustCommand\vdots{\mathpalette\@vdots{}}
\newcommand*{\@vdots}[2]{%
	% #1: math style
	% #2: unused
	\sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
	\sbox2{$#1.\m@th$}%
	\vbox{%
		\dimen@=\wd0 %
		\advance\dimen@ -3\ht2 %
		\kern.5\dimen@
		% remove side bearings
		\dimen@=\wd2 %
		\advance\dimen@ -\ht2 %
		\dimen2=\wd0 %
		\advance\dimen2 -\dimen@
		\vbox to \dimen2{%
			\offinterlineskip
			\copy2 \vfill\copy2 \vfill\copy2 %
		}%
	}%
}
\DeclareRobustCommand\ddots{%
	\mathinner{%
		\mathpalette\@ddots{}%
		\mkern\thinmuskip
	}%
}
\newcommand*{\@ddots}[2]{%
	% #1: math style
	% #2: unused
	\sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
	\sbox2{$#1.\m@th$}%
	\vbox{%
		\dimen@=\wd0 %
		\advance\dimen@ -3\ht2 %
		\kern.5\dimen@
		% remove side bearings
		\dimen@=\wd2 %
		\advance\dimen@ -\ht2 %
		\dimen2=\wd0 %
		\advance\dimen2 -\dimen@
		\vbox to \dimen2{%
			\offinterlineskip
			\hbox{$#1\mathpunct{.}\m@th$}%
			\vfill
			\hbox{$#1\mathpunct{\kern\wd2}\mathpunct{.}\m@th$}%
			\vfill
			\hbox{$#1\mathpunct{\kern\wd2}\mathpunct{\kern\wd2}\mathpunct{.}\m@th$}%
		}%
	}%
}
% \colon for maps in opposite direction (https://tex.stackexchange.com/a/2303/27717)
\newcommand*\noloc{%
	\nobreak
	\mskip6mu plus1mu
	\mathpunct{}%
	\nonscript
	\mkern-\thinmuskip
	{:}%
	\mskip2mu
	\relax
}
% Used for aligning math material
\newlength{\TmpLenA}
\newlength{\MBoxWidth}
\NewDocumentCommand{\MBox}{O{l}mO{\MBoxWidth}}{\mathmakebox[#3][#1]{#2}}
% like column types l, r, c, but without column spaces.
\newcolumntype{L}{@{} >{{}} l <{{}} @{} }
\newcolumntype{R}{@{} >{{}} r <{{}} @{} }
\newcolumntype{C}{@{} >{{}} c <{{}} @{} }
\newcolumntype{M}[1]{>{\centering\let\newline\\\arraybackslash}m{#1}}
% useful for alignment in algorithms
\newcommand{\Array}[3][c]{
	\begingroup
	\def\;{\\}
	\begin{array}[#1]{#2}
		#3
	\end{array}
	\endgroup
}
% END_FOLD
% BEGIN_FOLD Theorems
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newenvironment{theoremmbis}{%
	\NextLinkTarget{theorem.\thetheorem.bis}%
	\addtocounter{theorem}{-1}%
	\let\origthetheorem\thetheorem
	\renewcommand{\thetheorem}{\origthetheorem$'$}%
	\begin{theorem}%
}{%
	\end{theorem}
}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{construction}[theorem]{Contruction}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

% END_FOLD
% BEGIN_FOLD TikZ
\usetikzlibrary{calc,shapes,shapes.misc,backgrounds,cd}
\input{modules}
\tikzset{%
	on layer/.code={\pgfonlayer{#1}\begingroup\aftergroup\endpgfonlayer\aftergroup\endgroup},
	sans small/.style={
		every label/.append style={font={\scriptsize\mathversion{sans}\sffamily}},
		every node/.append style={font={\scriptsize\mathversion{sans}\sffamily}}
	},
	module diagram/.append style={sans small},
	math node/.style={execute at begin node=$#1, execute at end node=$},
	math node/.default=\textstyle,
	caption/.style={below=0pt of current bounding box, math node},
}
\tikzcdset{%
	tilted diagram/shift/.initial=3.5em,
	tilted diagram/column sep/.initial=7em,
	tilted diagram/even row sep/.initial=2.75em,
	tilted diagram/odd row sep/.initial=2.25em,
	tilted diagram/.style={
		column sep={\pgfkeysvalueof{/tikz/commutative diagrams/tilted diagram/column sep},between origins},
		/tikz/every even row/.append style={
			row sep={\pgfkeysvalueof{/tikz/commutative diagrams/tilted diagram/even row sep},between origins}
		},
		/tikz/every odd row/.append style={
			xshift=\pgfkeysvalueof{/tikz/commutative diagrams/tilted diagram/shift},
			row sep={\pgfkeysvalueof{/tikz/commutative diagrams/tilted diagram/odd row sep},between origins}
		}
	}
}
% END_FOLD
% BEGIN_FOLD Bibliography
\addbibresource{submission.bib}
\renewcommand*{\multicitedelim}{\addsemicolon\space}
\AtEveryBibitem{%
	\clearfield{eventtitle}%
	\clearfield{venue}%
	\clearfield{eventyear}%
	\iffieldundef{doi}{}{%
		\clearfield{issn}%
		\clearfield{isbn}%
		\clearfield{url}%
	}%
}
% END_FOLD

\newcommand{\newlinearrowleftlooseness}{2}
\newcommand{\newlinearrowrightlooseness}{2}
\NewDocumentCommand{\newlinearrow}{
	O{0pt} % additional line skip
	m % label left curve
	O{0pt} % shift horizontal part of arrow up/down
	m % label right curve
	O{->}
}{
	% Save coordinate where arrow starts.
	\mathrel{\tikz[remember picture, baseline=0] \path (0,0.5ex) coordinate (A);}
	% Insert newline
	{} \\[#1] {}
	% Draw the arrow
	\mathrel{
		\tikz[remember picture, overlay, baseline=0, auto]\draw[#5]
		(0,0.6ex) coordinate (B) % startpoint
		($(A)!0.5!(B) + (0,#3)$) coordinate (C) % point in the middle of horizontal part
		(C -| A) coordinate (D) % end point of the right loop
		(C -| B) coordinate (E) % end point of left loop
		(A) to[out=0, in=0, looseness=2] node{$\scriptstyle #4$} (D) to (E)
		to[out=180, in=180, looseness=2] node[swap] {$\scriptstyle #2$} (B);
	}
}

\usepackage{siunitx}
\sisetup{group-minimum-digits=4, detect-family}
\newcolumntype{F}[1]{S[table-format={#1}]}
\newcolumntype{I}[1]{S[table-format={#1}, round-precision=0,round-mode=places]}

\DeclareFontShape{T1}{cmr}{m}{scit}{<->ssub*cmr/m/scsl}{} % Uses slanted instead of italic small caps

\makeatletter
\newcommand*{\Boldmath}{%
	\ifx\f@series\my@test@bf
		\boldmath
	\fi
}
\newcommand*{\my@test@bf}{bx}
\makeatother

